Automated Summarization of Stack Overflow Posts

Software developers often resort to Stack Overflow (SO) to fill their programming needs. Given the abundance of relevant posts, navigating them and comparing different solutions is tedious and time-consuming. Recent work has proposed to automatically summarize SO posts to concise text to facilitate the navigation of SO posts. However, these techniques rely only on information retrieval methods or heuristics for text summarization, which is insufficient to handle the ambiguity and sophistication of natural language. This paper presents a deep learning based framework called ASSORT for SO post summarization. ASSORT includes two complementary learning methods, ASSORT_S and ASSORT_{IS}, to address the lack of labeled training data for SO post summarization. ASSORT_S is designed to directly train a novel ensemble learning model with BERT embeddings and domainspecific features to account for the unique characteristics of SO posts. By contrast, ASSORT_{IS} is designed to reuse pre-trained models while addressing the domain shift challenge when no training data is present (i.e., zero-shot learning). Both ASSORT_S and ASSORT_{IS} outperform six existing techniques by at least 13% and 7% respectively in terms of the F1 score. Furthermore, a human study shows that participants significantly preferred summaries generated by ASSORT_S and ASSORT_{IS} over the best baseline, while the preference difference between ASSORT_S and ASSORT_{IS} was small.

==> data_collection.tex <==
\section{data collection}
\todo{We (I changed the subject because I expect to get more posts from the interns)} manually curated summaries of 2278 popular SO answer posts and construct a dataset named \dataset. This section describes the process of dataset construction. 

%\noindent\setlength{\parskip}{0.3em}
\subsection{SO Post Pre-processing}
\todo{We first ranked all SO questions with the Stack Overflow online explorer based on their view counts. We chose view counts since we wanted to focus on popular SO posts first.}
%We first extracted SO questions from the Stack Overflow data dump~\cite{sodatadump} and ranked them based on their view counts. We chose view counts since we wanted to focus on popular SO posts first. 
Then, the first author manually inspected the frequently viewed questions and selected three types of commonly asked questions---{\howto} questions, {\whatis} questions, and {\debug} questions identified by prior work~\cite{treude2011programmers, question_type}. Eventually, the first author selected 177 {\howto}, 182 {\whatis}, and 147 {\debug} questions to form a balanced dataset. 
\todo{We took every answer post under the 506 questions except the ones with negative scores with the intention to control post quality in the dataset. We also removed answer posts that only contain code snippets as code summarization is not the focus of this work.}
%For each question post, we filtered out its answer posts with negative scores since they may not be valid answers. We also removed answer posts that only contain code snippets. 
For the remaining 2,283 answer posts, we extracted their content and other metadata such as view counts and post scores from the SO data dump.
\todo{We preprocess the content of the answer posts by removing the HTML tags and break them into sentences with the NLTK package.}
%Since the content of each post was stored as plain HTML in the data dump, we removed the HTML tags and used the NLTK package~\cite{nltk} to break natural language descriptions into sentences. Pre-processed question posts and answer posts were stored in CSV.

\subsection{SO Post Labeling Pipeline}


We followed the common standard of NLP data labeling process to label SO posts~\cite{xu2020review, rodrigues2014sequence, boujou2021open}. The first two authors first independently labeled summative sentences in 464 answer posts from the first 100 questions in the dataset. 
\todo{The authors meet to compare their labeling results which give an initial Cohen's kappa score of 0.41}
%Then, the authors compared their labeling results and resolved the inconsistencies. The initial Cohen's kappa score is 0.41. 
During the discussion, a set of labeling rules were summarized to mitigate bias and ensure labeling consistency. 
Based on these labeling rules, the first two authors labeled 526 posts from the second batch of 100 questions in the dataset. The authors met again and compared their labeling results. The kappa score of the second-round labeling is increased to 0.67, which indicates a moderate agreement under the guidance of the labeling rules~\cite{mchugh2012interrater}. The authors resolved some inconsistencies and further refined the labeling rules. 
Finally, they continued to label the rest 1288 answer posts and resolved inconsistencies. %The final kappa score for all 506 questions is 0.63. 
The final SOSum dataset only includes summative sentences that both authors agree upon. This whole labeling process takes about 175 man-hours.

The final set of labeling rules are summarized below.

\noindent{\bf\em Prefer sentences that directly answer a question.} For example, in Figure~\ref{table:example}, sentence 1-3 all contribute to the post on a high level but since the question asks for the difference between visibility:hidden and display:none, we select sentence 2 and 3.

\noindent{\bf\em Prefer topic sentences over illustrative descriptions.} Sentences such as ``for example,...'' are not preferred, while sentences that describe a high-level concept or idea are preferred. 
    
\noindent{\bf\em Prefer instructions over explanations}
    Sentences with clear instructions on how to complete a programming task or fix a bug, if any, are selected. Sentences explaining these instructions are not.
    
\noindent{\bf\em Select a complete list of items or steps.} If one sentence in a bullet list or procedure (e.g. \emph{``First, try A. Then, do B.''}) is selected, the corresponding sentences for the following items or steps should also be selected to ensure completeness and consistency.

\noindent{\bf\em Prefer concise sentences over verbose sentences.} If there are two summative sentences, we always pick the shorter one.

\setlength{\parskip}{0em}


==> threat.tex <==
\section{Threat to validity}
